The exploration-exploitation paradigm: a biophysical approach

This PhD thesis is essentially the story of a scientific idea, from what it has blossomed, how it has grown, what it might become. My ambition in writing has been to produce an original, coherent and compact narrative. It begins (1) with a discussion of the meaning, ambitions and circumstances of biological physics, as I understand them. Two background chapters discuss (2) the maxent inference by exponential random graph (ERG) models and (3) a theoretical approach to evolutionary dynamics. By generalising the evolutionary problem, the exploration-exploitation (EE) problem for biological dynamics is formalised and studied analytically in toy models (4). It is then used to tackle the brain wiring problem, focusing on the maturation of the C. elegans connectome (5). It is shown that a parsimonious ERG description of the adult worm brain combined with EE dynamics is able to trace the entire developmental trajectory.

==> chapters/coda.tex <==
\chapter*{Coda: beyond this manuscript}
\addcontentsline{toc}{chapter}{Coda} 

%\chapter{Wrong ideas, dead ends}
%\addcontentsline{toc}{chapter}{Wrong ideas, dead ends} 
